Understanding Clipping for Federated Learning: Convergence and Client-Level Differential Privacy

Providing privacy protection has been one of the primary motivations of Federated Learning (FL). Recently, there has been a line of work on incorporating the formal privacy notion of differential privacy with FL. To guarantee the client-level differential privacy in FL algorithms, the clients' transmitted model updates have to be clipped before adding privacy noise. Such clipping operation is substantially different from its counterpart of gradient clipping in the centralized differentially private SGD and has not been well-understood. In this paper, we first empirically demonstrate that the clipped FedAvg can perform surprisingly well even with substantial data heterogeneity when training neural networks, which is partly because the clients' updates become similar for several popular deep architectures. Based on this key observation, we provide the convergence analysis of a differential private (DP) FedAvg algorithm and highlight the relationship between clipping bias and the distribution of the clients' updates. To the best of our knowledge, this is the first work that rigorously investigates theoretical and empirical issues regarding the clipping operation in FL algorithms.

==> app_v2.tex <==
\subsection{Proof of Theorem \ref{thm: fedavg_conv}}
By Lipschitz smoothness, we have 
\begin{align}
    f(x_{t+1}) \leq f(x_t) + \langle \nabla f(x_t), x_{t+1} - x_t \rangle + \frac{L}{2} \|x_{t+1} - x_t\|^2
\end{align}
Before we proceed, we define following quantities to simplify notation.
\begin{align}
&\alpha_i^t = \frac{c}{\max(c,\eta_l \|\sum_{q=0}^{Q-1} g_i^{t,q} \|)}, \quad 
\tilde \alpha_i^t = \frac{c}{\max(c,\eta_l  \| \mathbb E[ \sum_{q=0}^{Q-1} g_i^{t,q} ]\|)},  \quad 
\overline \alpha^t = \frac{1}{N} \sum_{i=1}^N \tilde \alpha_i^t, \nonumber \\
&\Delta_i^t = -\eta_l \sum_{q=0}^{Q-1} g_i^{t,q} \cdot \alpha_i^t , \quad
\tilde \Delta_i^t = -\eta_l \sum_{q=0}^{Q-1} g_i^{t,q} \cdot \tilde \alpha_i^t, \nonumber \\
&\overline \Delta_i^t = -\eta_l \sum_{q=0}^{Q-1} g_i^{t,q} \cdot \overline \alpha^t  \quad \breve  \Delta_i^t = -\eta_l \sum_{q=0}^{Q-1} \nabla f(x_i^{t,q}) \cdot \overline \alpha^t  
\end{align}
where the expectation in $\tilde \alpha_i^t$ is taken over all possible randomness.

Then we have $x_{t+1} - x_t = \eta_g \frac{1}{N} \sum_{i=1}^N (\Delta_i^t + z_i^t)$ with $z_i^t \sim \mathcal N (0, \sigma^2 I)$ and conditioned on $x_t$,
\begin{align}\label{eq: lip}
    \mathbb E [f(x_{t+1})] \leq f(x_t)  + \eta_g {\left\langle \nabla f(x_t), \mathbb E\left[\frac{1}{N} \sum_{i=1}^N \Delta_i^t\right] \right\rangle} + \frac{L}{2} \eta_g^2 \mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N \Delta_i^t \right\|^2\right] + \frac{L}{2} \eta_g^2 \frac{1}{N} \sigma^2 d 
\end{align}
The next steps will analyze the bias caused by clipping by looking at the first order term. We have
\begin{align}\label{{eq: bias_split}}
   & \left\langle \nabla f(x_t), \mathbb E\left[\frac{1}{N} \sum_{i=1}^N \Delta_i^t\right] \right\rangle \nonumber \\
= & \left\langle \nabla f(x_t), \mathbb E\left[\frac{1}{N} \sum_{i=1}^N \Delta_i^t - \tilde \Delta_i^t \right] \right\rangle  + \left\langle \nabla f(x_t), \mathbb E\left[\frac{1}{N} \sum_{i=1}^N \tilde \Delta_i^t - \overline \Delta_i^t\right] \right\rangle  \nonumber \\
& +  \left\langle \nabla f(x_t), \mathbb E\left[\frac{1}{N} \sum_{i=1}^N \overline \Delta_i^t\right] \right\rangle 
\end{align}
where the first two terms of RHS of the above equality can be viewed as bias caused by clipping. The first order predicted descent can be analyzed from the last term by completing the square.
\begin{align}
   & \left\langle \nabla f(x_t), \mathbb E\left[\frac{1}{N} \sum_{i=1}^N \overline \Delta_i^t\right] \right\rangle  \nonumber \\
   = & \mathbb  E\left[ \left\langle \nabla f(x_t), \frac{1}{N} \sum_{i=1}^N \breve \Delta_i^t\right] \right\rangle  \nonumber \\
   =& \frac{-\eta_l \overline \alpha^t Q}{2} \|\nabla f(x_t)\|^2 -  \frac{\eta_l\overline \alpha^t}{2Q} \mathbb E \left[ \left\| \frac{1}{\eta_l N \overline \alpha^t} \sum_{i=1}^N \breve \Delta_i^t\right\|^2\right] \nonumber \\
  &+ \frac{\eta_l \overline \alpha^t}{2}  \underbrace{ \mathbb E \left[\left\|\sqrt{Q} \nabla f(x_t) - \frac{1}{\sqrt{Q}} \frac{1}{\eta_l N \overline \alpha^t}  \sum_{i=1}^N \overline \Delta_i^t\right \|^2 \right]}_{A_1}
\end{align}
We further upper bound $A_1$ as
\begin{align}\label{eq: A1}
    A_1  
    = & Q  \mathbb E \left[\left \| \nabla f(x_t) - \frac{1}{{Q}N} \sum_{i=1}^N \sum_{q=0}^{Q-1} \nabla f_i(x_i^{t,q}) \right \|^2\right] \nonumber \\
    =  & Q  \mathbb E \left[\left \|   \frac{1}{{Q}N} \sum_{i=1}^N \sum_{q=0}^{Q-1} \nabla f_i(x^t) -  \nabla f_i(x_i^{t,q})  \right \|^2 \right] \nonumber \\
    \leq & \frac{1}{N} \sum_{i=1}^N \sum_{q=0}^{Q-1} \mathbb E [ \| \nabla f_i(x^t) - \nabla f_i(x_i^{t,q}) \|^2 ]  \nonumber \\
    \leq & \frac{1}{N} \sum_{i=1}^N \sum_{q=0}^{Q-1} L^2 \mathbb E [ \|  x^t - x_i^{t,q} \|^2 ]  \nonumber \\
    \leq & L^2 5 Q^2 \eta_l^2 (\sigma_l^2 + 6Q \sigma_g^2) + L^2 30 Q^3 \eta_l^2 \|\nabla f(x_t)\|^2
\end{align}
where the last inequality is due to \cite{}[a lemma in Yang et al., 2021 and Reddi et al., 2021].

Now we turn to upper bounding the second order term in \eqref{eq: lip}.
\begin{align}\label{eq: second_term}
     & \mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N \Delta_i^t \right\|^2\right] \nonumber \\ 
     \leq & 3 \mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N \Delta_i^t - \tilde \Delta_i^t \right\|^2\right] + 3 \mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N \tilde \Delta_i^t - \overline \Delta_i^t  \right\|^2\right] + 3 \mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N  \overline \Delta_i^t  \right\|^2\right] \nonumber \\
 %    \leq & 3 \mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N \Delta_i^t - \tilde \Delta_i^t \right\|^2\right] + 3 \mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N \tilde \Delta_i^t - \overline \Delta_i^t  \right\|^2\right] + 3 \mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N \mathbb E[ \overline \Delta_i^t ] \right\|^2\right] + \frac{3 Q\eta_l^2 (\overline  \alpha^t)^2 \sigma_l^2}{N}
\end{align}
For the last term in \eqref{eq: second_term}, we have 
\begin{align}\label{eq: split_variance}
    &\mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N \overline \Delta_i^t \right\|^2\right]  \nonumber \\
    = & \mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N -\eta_l \sum_{q=0}^{Q-1} g_i^{t,q} \cdot \overline \alpha^t \right\|^2\right] \nonumber \\
    \leq & \mathbb E \left [ 2 \left \|\frac{1}{N} \sum_{i=1}^N -\eta_l \sum_{q=0}^{Q-1} \nabla f(x_i^{t,q}) \cdot \overline \alpha^t \right\|^2 + 2 \left \|\frac{1}{N} \sum_{i=1}^N -\eta_l \sum_{q=0}^{Q-1} (\nabla f(x_i^{t,q}) -g_i^{t,q}) \cdot \overline \alpha^t \right\|^2\right] \nonumber \\
    = & 2 \mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N \breve \Delta_i^t \right\|^2\right] + \frac{2}{N}\eta_l^2\overline \alpha^2 Q \sigma_l^2
\end{align}

Combining \eqref{eq: lip}-\eqref{eq: second_term}, we have
\begin{align}
        \mathbb E [f(x_{t+1})] \leq & f(x_t)  + \frac{-\eta_g\eta_l \overline \alpha^t Q}{2} \|\nabla f(x_t)\|^2 - \frac{\eta_g\eta_l\overline \alpha^t}{2Q} \mathbb E \left[ \left\| \frac{1}{\eta_l N \overline \alpha^t} \sum_{i=1}^N \breve \Delta_i^t\right\|^2\right] \nonumber \\
  &+ \frac{\eta_g\eta_l \overline \alpha^t}{2} (5L^2  Q^2 \eta_l^2 (\sigma_l^2 + 6Q \sigma_g^2) + 30L^2  Q^3 \eta_l^2 \|\nabla f(x_t)\|^2) \nonumber \\
        &+ \eta_g \left\langle \nabla f(x_t), \mathbb E\left[\frac{1}{N} \sum_{i=1}^N \Delta_i^t - \tilde \Delta_i^t \right] \right\rangle  + \eta_g \left\langle \nabla f(x_t), \mathbb E\left[\frac{1}{N} \sum_{i=1}^N \tilde \Delta_i^t - \overline \Delta_i^t\right] \right\rangle \nonumber \\
        & + 3L\eta_g^2 \mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N \breve \Delta_i^t \right\|^2\right]  +  \frac{3L}{N}\eta_g^2\eta_l^2(\overline \alpha^t)^2 Q \sigma_l^2 + \frac{L}{2} \eta_g^2 \frac{1}{N} \sigma^2 d   \nonumber \\
        & + \frac{3L}{2} \eta_g^2 \mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N \Delta_i^t - \tilde \Delta_i^t  \right\|^2\right]  + \frac{3L}{2} \eta_g^2 \mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N \tilde\Delta_i^t -  \overline\Delta_i^t  \right\|^2\right]  
\end{align}
When $\eta_g\eta_l \leq \frac{1}{6QL}$ and $\eta_l \leq \frac{1}{\sqrt{60}QL}$, the above inequality simplifies to 
\begin{align}
    \mathbb E [f(x_{t+1})] 
    \leq & f(x_t)  + \frac{-\eta_g\eta_l \overline \alpha^t Q}{4} \|\nabla f(x_t)\|^2  \nonumber \\
  &+ \frac{\eta_g\eta_l^3 \overline \alpha^t}{2} (5L^2  Q^2  (\sigma_l^2 + 6Q \sigma_g^2)) \nonumber \\
        &+ \eta_g \left\langle \nabla f(x_t), \mathbb E\left[\frac{1}{N} \sum_{i=1}^N \Delta_i^t - \tilde \Delta_i^t \right] \right\rangle  + \eta_g \left\langle \nabla f(x_t), \mathbb E\left[\frac{1}{N} \sum_{i=1}^N \tilde \Delta_i^t - \overline \Delta_i^t\right] \right\rangle \nonumber \\
        & + \frac{3L}{N}\eta_g^2\eta_l^2(\overline \alpha^t)^2 Q \sigma_l^2 + \frac{L}{2} \eta_g^2 \frac{1}{N} \sigma^2 d   \nonumber \\
        & + \frac{3L}{2} \eta_g^2 \mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N \Delta_i^t - \tilde \Delta_i^t  \right\|^2\right]  + \frac{3L}{2} \eta_g^2 \mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N \tilde\Delta_i^t -  \overline\Delta_i^t  \right\|^2\right]  
\end{align}
Sum over $t$ from $1$ to $T$, divide both sides by $T\eta_g\eta_lQ/4$, and rearrange, we have
\begin{align}
      &\frac{1}{T} \sum_{t=1}^T \mathbb E[ \overline \alpha^t\|\nabla f(x_t)\|^2] \nonumber \\
    \leq & \frac{4}{T\eta_g\eta_lQ}(\mathbb E [f(x_{1})] -  \mathbb E [f(x_{T+1})])      \nonumber \\
  &+ {10\eta_l^2 } L^2  Q  (\sigma_l^2 + 6Q \sigma_g^2) \frac{1}{T}\sum_{t=1}^T \overline \alpha^t + \frac{12L}{N}\eta_g\eta_l  \sigma_l^2 \frac{1}{T}\sum_{t=1}^T (\overline \alpha^t)^2+  2L\frac{ \eta_g}{\eta_lQN} d \sigma^2    \nonumber \\
        &+ \frac{1}{T}\sum_{t=1}^T \frac{4}{\eta_lQ} \mathbb E\left[\left\langle \nabla f(x_t), \mathbb E\left[\frac{1}{N} \sum_{i=1}^N \Delta_i^t - \tilde \Delta_i^t \right] \right\rangle  + \left\langle \nabla f(x_t), \mathbb E\left[\frac{1}{N} \sum_{i=1}^N \tilde \Delta_i^t - \overline \Delta_i^t\right] \right\rangle \right ] \nonumber \\
        & + \frac{6L}{\eta_lQ} \eta_g \frac{1}{T} \sum_{t=1}^T \mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N \Delta_i^t - \tilde \Delta_i^t  \right\|^2\right]  + \frac{6L}{\eta_lQ} \eta_g \frac{1}{T} \sum_{t=1}^T \mathbb E \left [\left \|\frac{1}{N} \sum_{i=1}^N \tilde\Delta_i^t -  \overline\Delta_i^t  \right\|^2\right].  
\end{align}
Upper-bounding the last four terms using $\|g_i^{t,q}\| \leq G$ yields the desired result. \qed

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

